Accelerating Training of Transformer-Based Language Models with Progressive Layer Dropping

Recently, Transformer-based language models have demonstrated remarkable performance across many NLP domains. However, the unsupervised pre-training step of these models suffers from unbearable overall computational expenses. Current methods for accelerating the pre-training either rely on massive parallelism with advanced hardware or are not applicable to language modeling. In this work, we propose a method based on progressive layer dropping that speeds the training of Transformer-based language models, not at the cost of excessive hardware resources but from model architecture change and training technique boosted efficiency. Extensive experiments on BERT show that the proposed method achieves a 24% time reduction on average per sample and allows the pre-training to be 2.5 times faster than the baseline to get a similar accuracy on downstream tasks. While being faster, our pre-trained models are equipped with strong knowledge transferability, achieving comparable and sometimes higher GLUE score than the baseline when pre-trained with the same number of samples.

==> ack.tex <==
\begin{ack}
The authors are grateful for the useful discussion with Xiaodong Liu, and Wenhan Wang. 
The authors appreciate the anonymous NeurIPS reviewers for providing constructive feedback for improving the quality of this paper. All authors are not funded by any other agency.
\end{ack}

==> additional.tex <==
\section{Model Architecture Change For Layer-Drop}

One natural way to increase the model capacity is simply increasing the layer number $L$. Unfortunately, Figure~\ref{fig:vanishing-gradients} shows that this would raise gradient vanishing issue at the lower layers. When $L=12$, which is the default layer in the original BERT paper, the gradient vanishing issue exists, but is not severe. However, as we stack more Transformer encoder blocks, the vanishing gradient issue becomes significantly worse. The gradients at the bottom layers are so close to 0 that the learning at those layers becomes close to halt. 


% Simply increasing the depth of the model leads to vanishing gradient issue. 

\subsubsection{Revisiting the Transformer networks}

We define Transformer networks as the composition of Transformer blocks, where all Transformer blocks have the same architecture. In particular, a Transformer block consists of two sublayers: a dot-product self-attention layer and a feed-forward layer, with both layers having a skip connection. 
More concretely, for an input $X \in \mathds{R}^{d \times n}$ consisting of d-dimensional embeddings of $n$ tokens, a Transformer block consists of the following two sublayers:

% \begin{equation}
%     Attn(X) = X + \sum_{i=1}^{h}{W_O^i}{W_V^i}X\cdot\sigma[(W_K^iX)^TW_Q^iX] 
% \end{equation}

\begin{equation}
\label{eqn:transformer-self-attention}
\begin{split}
    SL_1(X) &= LayerNorm(X + Attn(X)) \\
            &= LayerNorm(X + {W_O}{W_V}X\cdot softmax[(W_KX)^TW_QX])
\end{split}
\end{equation}

% where $W_O \in \mathds{R}^{}$

% \begin{equation}
%     FF(X) = Attn(X) + W_2\cdot GeLU(W_1\cdot Attn(X) + b_1) + b_2
% \end{equation}

\begin{equation}
\label{eqn:feed-forward}
\begin{split}
    SL_2(X) &= LayerNorm(SL_1(X) + FF(SL_1(X))) \\
            &= LayerNorm(SL_1(X) + W_2\cdot gelu(W_1\cdot SL_1(X)))
\end{split}
\end{equation}

Based on Eqn.~\ref{eqn:transformer-self-attention}--\ref{eqn:feed-forward}, we have for each layer $l$:

\begin{equation}
\label{eqn:analysis-1}
\begin{split}
    X_{l+1} &= LayerNorm(SL_1(X_l) + FF(SL_1(X_l))) \\
            &= LayerNorm(LayerNorm(X_{l} + Attn(X_{l})) + FF(LayerNorm(X_{l} + Attn(X_{l})))) \\
\end{split}
\end{equation}

% Assume $F(X, W) = {W_O}{W_V}X\cdot softmax[(W_KX)^TW_QX]$, then 
% Recursively we will have

% \begin{equation}
% \begin{split}
%     X_{l+2} &= LayerNorm(LayerNorm(X_{l+1} + Attn(X_{l+1})) + FF(LayerNorm(X_{l+1} + Attn(X_{l+1})))) \\
%     & = LayerNorm(LayerNorm(X_{l+1} + F(X_{l+1}))+ W_2(l)\cdot gelu(W_1(l)\cdot LayerNorm(X_{l+1} + F(X_{l+1}))) \\
%     & = ...
% \end{split}
% \end{equation}

% \begin{equation}
% \begin{split}
%     X_{l+2} &= LayerNorm(Attn(X_{l+1}) + W_2(l)\cdot gelu(W_1(l)\cdot Attn(X_{l+1}))) \\
%     & = LayerNorm(LayerNorm(X_{l+1} + F(X_{l+1}))+ W_2(l)\cdot gelu(W_1(l)\cdot LayerNorm(X_{l+1} + F(X_{l+1}))) \\
%     & = ...
% \end{split}
% \end{equation}

% Explain what LayerNorm is used for.



The layer normalization as in \cite{layer-norm} keeps the magnitude of the hidden layers from growing large. As can be seen, the LayerNorm layer alters the signal that passes through the skip connection and impedes information propagation, as reflected by the difficulties on reducing training loss after we increase the model depth (Fig.~\ref{}). Furthermore, SGD and dropout perturb the normalisation, leading to high variance in training error. The effect gets worse with depth, so simply stacking more Transformer blocks tend to perform poorly.

Explain why LayerNorm causes an issue.



% The encoder block passes the input features to a self-attention layer followed by a feed-forward neural network with 1 hidden layer and the ReLU activation function. Before these sub-modules, we follow the original work to include residual connections which establishes short-cuts between the lower-level representation and higher layers. The presence of the residual layers massively increases the magnitude of the neuron values is then alleviated by the layer-normalization layers placed after each residual connection. 




\href{https://arxiv.org/pdf/1911.03179.pdf}{Why Deep Transformers are Difficult to Converge?
From Computation Order to Lipschitz Restricted Parameter Initialization}

"We empirically show
that with proper parameter initialization, deep
Transformers with the original computation order can converge, which is quite in contrast
to all previous works, and obtain significant
improvements with up to 24 layers."

Plot: Gradient norm (y-axis) of each encoder layer (top)
and decoder layer (bottom) in Transformer with respect to layer depth (x-axis).

Show the difference between L12, L24, L48, L72, L101

1. By adding identity mapping, the output x can be thought of as a recursive summation of the outputs from all previous layers. In contrast, without skip connections, then the output is the products of a series of matrix-vector.

2. Gradients at skip connection boundary can be decomposed into two additive terms: a term that propagates information directly without concerning any weight layers, and another term that propagates through the weight layers. The first term ensures that the information is directly propagated back to any shallower unit. 
Another hypothesis is that the second term makes it more unlikely to have vanished gradients (this remains unclear as whether gradients indicate vanish in early layers in BERT, something to verify and potentially can be used to show if skip connections help).

3. Even though additional gating and conv shortcut introduces more parameters and should have a stronger representational abilities than identity shortcuts. Representation ability is not the only factor that decides whether a model behave good or not. There are at least two aspects: optimization issues and representational abilities. 

4. If additional components such as BN are added along the shortcut link, signals are altered before passing to previous layers (which indicates that we should keep the highway clean). 

5. Using asymmetric after-addition activation is equivalent to constructing a pre-activation Residual Unit.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figs/preln-improve-lr}
    \caption{Identity mapping reordering makes training more stable and helps the model to learn with a larger learning rate.}
    \minjia{Add learning rate schedules.}
    \minjia{Add changes of gradient norm before and after identity mapping and with different learning rate. We need fine-grained features to show that "identity mapping has an effect on stabilizing network parameters". Another way is to show the L2 distance and cosine similarity of the input and output embeddings for each layer. Check how Albert shows it with weight sharing.}
    \label{fig:preln-improve-lr}
\end{figure}

==> broader-impact.tex <==
\section*{Broader Impact}

% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

Pre-training large-scale language models like BERT have an incredible ability to extract textual information and apply to a variety of NLP tasks, but pre-training requires significant compute and time. Pre-training the BERT baseline model is typically done through hardware acceleration and scaling the training on 100s to 1000s of GPUs across multiple nodes. However, such a method is very costly and consumes magnitudes higher energy.

The proposed solution achieves similar or better quality with shorter training time. It improves robustness to further reduce the hyperparameter tuning required, improving the productivity of AI scientists. It also saves hardware resources and trims down the total energy cost of in-situ, resource-constrained training, yielding a less amount of carbon footprint produced. Furthermore, the optimizations not only benefit BERT; they are also applicable to many other recent models such as RoBERTa~\cite{roberta}, GPT-2~\cite{gpt-2}, XLNet~\cite{xlnet}, and UniLM~\cite{unilm}, which all adopt Transformer as the backbone. Finally, our techniques can also help advance language understanding and inference, enabling enterprise or consumer-facing applications, such as conversational AI. We will open-source the code so that other practitioners and researchers can reproduce our results or re-use code into their ventures in this field. 

There are no apparent negative outcomes. However, like other AI technology, we should be mindful of using it to transform our systems to be more efficient in fulfilling goodwill.     



==> related.tex <==
\section{Related Work}
\label{sec:related}

Our approach is a form of Dropout~\cite{dropout} applied to model layers instead of activation. Closer to our work, the Stochastic Depth approach drops layers randomly during training~\cite{stochastic-depth}. As opposed to our work, they are interested in accelerating the training of very deep ResNets in image recognition domain~\cite{resnet}, and they use a fixed dropping schedule for that goal. In contrast, we fill the gap by applying architectural change to the Transformer blocks first to stabilize the training and then introducing a progressive layer-drop schedule that takes into BERT training characteristics into account, shedding lights on this particular setting. Recent studies applied stochastic depth to train very deep Transformers for speech, but its goal is mostly to show the benefits of its regularization effect. 

More generally, our method is a form of structured pruning~\cite{structure-pruning}, which removes coherent groups of weights to preserve the original structure of the network. However, it is mostly adopted for compressing the model for efficient inference, whereas we focus on accelerating the training. 

% \subsection{Stochastic depth}

\href{https://www.kdnuggets.com/2016/04/stochastic-depth-networks-accelerate-deep-learning.html}{Stochastic Depth Networks Accelerate Deep Network Training}

% Prior work, Chen et al. (\cite{deep-transformer}) finds that pre-norm residual
% units (PRENORM), where layer normalization occurs immediately before the sublayer, are instrumental to their model’s performance. Wang et al.
% (2019) compare the two, showing that PRENORM
% makes backpropagation more efficient over depth and training Transformers with deep, 30-layer encoders. This is because it is equivalent to recasting LayerNorm as the pre-norm of the next Transformer block, and LayerNorm as pre-norm improves regularization of the models. 
% However, the deepest model they are able to train was 30-layer encoder model. In contrast, we demonstrate the effectiveness of more than 100-layer model.

\href{https://arxiv.org/pdf/1711.08393.pdf}{BlockDrop: Dynamic Inference Paths in Residual Networks}
